A Survey on the Honesty of Large Language Models

Honesty is a fundamental principle for aligning large language models (LLMs) with human values, requiring these models to recognize what they know and don't know and be able to faithfully express their knowledge. Despite promising, current LLMs still exhibit significant dishonest behaviors, such as confidently presenting wrong answers or failing to express what they know. In addition, research on the honesty of LLMs also faces challenges, including varying definitions of honesty, difficulties in distinguishing between known and unknown knowledge, and a lack of comprehensive understanding of related research. To address these issues, we provide a survey on the honesty of LLMs, covering its clarification, evaluation approaches, and strategies for improvement. Moreover, we offer insights for future research, aiming to inspire further exploration in this important area.

==> figures/outline.tex <==
\begin{figure*}[!t]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\normalsize,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=2pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            [
                A Survey on Honesty of Large Language Models,
                ver,
                color=hidden-draw,
                fill=mygray!30,
                text=black
                [
                    Honesty in LLMs, color=yellow!100, fill=yellow!100, text width=7.2em, text=black
                    [
                        What is Honesty, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                            [
                                Self-knowledge, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            ]
                            [
                                Self-Consistency, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                            ]
                    ]
                    [
                        Related Problems, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                        [
                            Hallucination, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{ji2023survey, zhang2023siren, huang2023survey, zhang2024knowledge, ji2024llm,liang2024learning}
                                \\
                                \cite{azaria2023internal,zhang2023language,liang2024learning,lu2024insights}
                            ]
                        ]
                        [
                            Unfaithful CoT, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{turpin2024language, lanham2023measuring, tanneru2024hardness,li2024towards}
                            ]
                        ]
                        [
                            Prompt Robustness, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{mizrahi2023state, shi2023large, gu2022robustness, wang2023robustness,sclar2024quantifying}
                            ]
                        ]
                        [
                            G-V Inconsistency, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{li2024benchmarking, jiang2024self, li2024benchmarking}
                            ]
                        ]
                        [
                            Over-confidence, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{mielke2022reducing,ling2024deductive, li2024think, khan2024debating, zhou2024relying, xu2024sayself}
                            ]
                        ]
                        [
                            Sycophancy, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{cotra2021ai,perez2022discovering,radhakrishnan2023question, wang2023can, khan2024debating, park2024ai}
                            ]
                        ]
                    ]
                    [
                        Related Application, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                        [
                            Hallucination Mitigation, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                            [
                                \cite{chen2024teaching, wan2024knowledge, liang2024learning}
                            ]
                        ]
                        [
                            RAG, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                            [
                                \cite{wang2023self, jiang2023active, ni2024llms, liu2024ctrla, yao2024seakr, cheng2024unified}
                            ]
                        ]
                        [
                            Language Agent, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                            [
                                \cite{liang2024introspective, mullen2024towards, han2024towards, hu2024uncertainty, yoffe2024debunc}
                            ]
                        ]
                        [
                            Model Cascading, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                            [
                                \cite{yue2023large, lu2024c, jung2024trust, gupta2024language, wang2024cascade}
                            ]
                        ]
                    ]
                ]
                [
                    Evaluation, color=yellow!100, fill=yellow!100, text width=7em, text=black
                    [
                        Self-knowledge, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                        [
                            Recognition of 
                            \\ Known/Unknown, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                            [
                                \cite{yin2023large,amayuelas2023knowledge,liang2024learning,liu2024examining,gao2024best,chern2024behonest}
                            ]
                        ]
                        [
                            Calibration, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{guo2017calibration,geng2024survey,xiong2023can,lyu2024calibrating,brier1950verification,naeini2015obtaining}
                                \\
                                \cite{nixon2019measuring,kull2019beyond}
                            ]
                        ]
                        [
                            Selective Prediction, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{tomani2024uncertainty,xu2024sayself,xiong2023can,geng2024survey,mahaut2024factual,ren2023self}
                                \\
                                \cite{vashurin2024benchmarking}
                            ]
                        ]
                    ]
                    [
                        Self-consistency, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                        [
                            Reference-based, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{yin2023large,amayuelas2023knowledge,chern2024behonest,cheng2024can,liang2024learning, gekhman2024does}
                            ]
                        ]
                        [
                            Reference-free, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{sclar2024quantifying,mizrahi2023state,chern2024behonest,zhu2023promptbench,cao2024worst,park2024ai}
                                \\ \cite{chern2024behonest,li2024benchmarking,chern2024behonest}
                            ]
                        ]
                    ]
                ]
                [
                    Improvement of \\ Self-knowledge, color=yellow!100, fill=yellow!100, text width=7em, text=black
                    [
                        Training-free, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                        [
                            Predictive Probability, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{adiwardana2020towards, malinin2020uncertainty, si2022prompting, kuhn2023semantic, kadavath2022language}
                                \\
                                \cite{ren2023self,duan2023shifting,achiam2023gpt}
                            ]
                        ]
                        [
                            Prompting, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{kadavath2022language,zhao2024fact,jiang2024self,yin2023large,tian2023just,wei2022chain}
                                \\
                                \cite{xiong2023can,zhou2023navigating}
                            ]
                        ]
                        [
                            Sampling and Aggregation, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{zhou2022prompt, kuhn2023semantic, lyu2024calibrating, xiong2023can, yang2024just,williams2018broad}
                                \\
                                \cite{lin2023generating, manakul2023selfcheckgpt, chen2024inside, huang2024calibrating, farquhar2024detecting, fadeeva2024fact}
                            ]
                        ]
                    ]
                    [
                        Training-based, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                        [
                            Supervised Fine-tuning, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{yang2023alignment, zhang2024r, cheng2024can, chen2024teaching, wan2024knowledge, kapoor2024large}
                                \\
                                \cite{lin2022teaching, ulmer2024calibrating, han2024enhancing}
                            ]
                        ]
                        [
                            Reinforcement Learning, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{cheng2024can,xu2024rejection,gao2024best,xu2024sayself,stengel2024lacie,band2024linguistic}
                            ]
                        ]
                        [
                            Probing, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{kadavath2022language,azaria2023internal,liu2024universal,ji2024llm,burns2023discovering,kossen2024semantic}
                            ]
                        ]
                    ]
                ]
                [
                    Improvement of \\ Self-consistency, color=yellow!100, fill=yellow!100, text width=7em, text=black
                    [
                        Training-free, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                        [
                            Chain-of-thought Prompting, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{wei2022chain,chenprogram, zhouleast, zheng2023take, wangexecutable}
                                \\
                                \cite{wanghypothesis, qiuphenomenal, yang2024language,zhou2023navigating,feng2024teaching}
                            ]
                        ]
                        [
                            Decoding-time Intervention, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{li2024inference, chen2024context, chuang2024dola, zhang2023alleviating, shi2024trusting, shi2024unchosen, leng2024mitigating}
                            ]
                        ]
                        [
                            Sampling and Aggregation, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{wang2023selfconsistency, chen2023universal, thirukovalluru2024atomic, wang2024integrate}
                            ]
                        ]
                        [
                            Post-generation Approaches, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{dhuliawala2023chain, varshney2023stitch, zhao2023verify}
                            ]
                        ]
                    ]
                    [
                        Training-based, color=yellow!100, fill=yellow!100, text width=9.0em, text=black
                        [
                            Self-aware Fine-tuning, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{yang2023alignment, zhang2024r, cheng2024can, wan2024knowledge}
                            ]
                        ]
                        [
                            Self-supervised Fine-tuning, color=yellow!100, fill=yellow!100, text width=9.8em, text=black
                            [
                                \cite{tian2024finetuning, zhang2024self, lin2024flame}
                            ]
                        ]
                    ]
                ]
                [
                    Future Work, color=yellow!100, fill=yellow!100, text width=7em, text=black
                    [
                        Evaluation
                    ]
                    [
                        Instruction-following Scenario.
                    ]
                    [
                        Honesty Regarding Input Context.
                    ]
                    [
                        Honesty Across Various Large Foundation Models.
                    ]
                ]
            ]   
        \end{forest}
    }
\caption{The outline of this survey.}
\label{outline}
\end{figure*}

==> section/application.tex <==
\subsection{Related Applications}
\label{sec:application_of_llm_honesty}



Honesty also plays a critical role in several scenarios, which we will explore in the following discussion.

\paragraph{Hallucination Detection and Mitigation.}
As discussed in \textsection\ref{sec-related-hallu}, the deficiency in honesty would lead to hallucination. 

There been many studies detect
Thus, we can check the ability of self-knowledge or self-expression to detect hallucination. Specifically, SelfCheckGPT \citep{manakul2023selfcheckgpt} detects hallucination on the assumption that stochastically sampled responses are likely to diverge, corresponding to the lack of self-consistency.
Also, \citet{fadeeva2024fact} detects hallucination via unreliable predictions based on the uncertainty scores, which is an application of self-knowledge.  
On the other hand, improving self-knowledge or self-consistency capability would help alleviate hallucinations.
To improve self-knowledge, the goal is to possess external factual knowledge \citep{wan2024knowledge} or better express the knowledge boundary \citet{chen2024teaching}.
% \citet{chen2024teaching} first collects training data based on the internal signals of the model and then trains the LLM with an additional loss of regularization to better express the knowledge boundary.
% Meanwhile, KCA \citep{wan2024knowledge} aims to align external knowledge encapsulated in alignment training data and intrinsic knowledge inherited in the pretraining corpus, which helps LLMs possess external factual knowledge.
% \citet{yoffe2024debunc} employ multi-agents to debate in multi-round, where the confidence of each agent would be synchronized in the next round. 
Moreover, \citet{liang2024learning} introduces model knowledge state assessments into the reinforcement learning feedback mechanism, aiming to encourage the model to rely on internal knowledge to answer (i.e., self-consistency) or honestly express its lack of relevant knowledge (i.e., self-knowledge).


\paragraph{Retrieval Augmented Generation.} 
Retrieval Augmented Generation~(RAG) aims to augment the generation results of LLMs based on the retrieval of relevant knowledge \citep{guu2020retrieval,yih2020retrieval,asai2023self}, showing promising performance to address hallucination \citep{shuster2021retrieval, magesh2024hallucination, lv2024coarse}.
However, invoking retrieval indiscriminately leads to various issues, including high retrieval costs \citep{zhao2024retrieval} and decreased performance due to poor retrieval results \citep{liu2024ra}.
Therefore, \textit{When to retrieve} becomes an important topic, where LLMs should retrieve if and only if they lack the required knowledge \citep{jiang2023active, liu2024ctrla}.
The key is to detect the knowledge boundary of LLMs, which is exactly the self-knowledge ability.
% Current mainstreaming methods to detect knowledge boundary can be categorized into 1) confidence-based and 2) self-knowledge-based.
SKR \citep{wang2023self} detects the knowledge boundary by building a corresponding dataset, which is time-consuming and model-specific.
FLARE~\citep{jiang2023active} employs an active retrieval strategy that only retrieves when LLMs generate low-probability tokens, based on the assumption that LLMs tend to be well calibrated and generate low confidence if they lack knowledge \citep{kadavath2022language}.
Due to the over-confidence issue, \citet{ni2024llms} propose three methods of prompting to urge LLMs to be prudent about their claims of certainty.
% and thus benefits adaptive retrieval augmentation.
Beyond the outputs, another way is to detect confidence based on the internal states \citep{liu2024ctrla, yao2024seakr}.
More recently, UAR \citep{cheng2024unified} unifies four orthogonal criteria to decide whether to retrieve, including intent-aware, knowledge-aware, time-sensitive-aware, and self-aware (i.e., self-knowledge). 

\paragraph{Language Agent.} 
The goal of language agent is to interact with the external world and solve tasks via LLMs \citep{xi2023rise,han2024towards}.
% However, the hallucination of LLMs would mislead users or cause tasks to fail.
When making a decision, an important principle is to possess a reliable mechanism to measure uncertainty of its own proposition or observations from the environment \citep{bacchus1996statistical}. 
To this end, it is vital to assess their confidence and then decide to execute the actions or ask an appropriate follow-up question to disambiguate \citep{liang2024introspective, mullen2024towards, han2024towards}.
Improving self-knowledge and self-consistency is crucial to assessing confidence.
Meanwhile, the criteria of the follow-up questions is to reduce uncertainty \citep{hu2024uncertainty}.
% Another way is to employ multi-agents to debate in multi-round, where the confidence of each agent would be synchronized in the next round \citep{yoffe2024debunc}.
% To assess the confidence, \citet{yoffe2024debunc} employ multi-agents to debate in multi-round, where the confidence of each agent would be synchronized in the next round.
% These methods are equivalent to improving the self-consistency and avoiding over-confidence. 


\paragraph{Model Cascading.} 
Typically, LLMs with better performance lead to higher costs than LLMs with relatively worse performance.
One solution is model cascading \citep{chen2023frugalgpt}, where inputs are first answered by a weaker LLM and only the hard cases are routed to a stronger LLM. 
The mainstreaming criterion for the router (a.k.a. deferral rule) is the confidence of the weaker LLM \citep{yue2023large, jung2024trust, gupta2024language, ramirez2024optimising}.
\citet{yue2023large} employ the sampling consistency to estimate confidence, which is consistent with our proposed self-consistency.
Meanwhile, calibrating the weak LLM is a promising approach \citep{lu2024c,jung2024trust}. 
In addition, \citet{gupta2024language} shows that the predicted sequence uncertainty suffers from the length bias problem, and thus design post hoc deferral rules using the quantiles over the uncertainty vector.
Furthermore, \citet{wang2024cascade} proposes cascade-aware training, using the average normalized log-likelihood to measure confidence.

% \paragraph{Decoding for Text Generation.}
% TBD
